The Future of High-Energy Astrophysical Neutrino Flavor Measurements

We critically examine the ability of future neutrino telescopes, including Baikal-GVD, KM3NeT, P-ONE, TAMBO, and IceCube-Gen2, to determine the flavor composition of high-energy astrophysical neutrinos, ie, the relative number of $\nu_e$, $\nu_\mu$, and $\nu_\tau$, in light of improving measurements of the neutrino mixing parameters. Starting in 2020, we show how measurements by JUNO, DUNE, and Hyper-Kamiokande will affect our ability to determine the regions of flavor composition at Earth that are allowed by neutrino oscillations under different assumptions of the flavor composition that is emitted by the astrophysical sources. From 2020 to 2040, the error on inferring the flavor composition at the source will improve from $> 40\%$ to less than $6\%$. By 2040, under the assumption that pion decay is the principal production mechanism of high-energy astrophysical neutrinos, a sub-dominant mechanism could be constrained to contribute less than 20\% of the flux at 99.7\% credibility. These conclusions are robust in the nonstandard scenario where neutrino mixing is non-unitary, a scenario that is the target of next-generation experiments, in particular the IceCube-Upgrade. Finally, to illustrate the improvement in using flavor composition to test beyond-the-Standard-Model physics, we examine the possibility of neutrino decay and find that, by 2040, combined neutrino telescope measurements will be able to limit the decay rate of the heavier neutrinos to below $1.8\times 10^{-5} (m/\mathrm{eV})$~s$^{-1}$, at 95\% credibility.

==> jdefs.tex <==
% Bibliography and bibfile
\def\pdu{Phys.\ Dark Univ.}
          % Physics of the Dark Universe
\def\lnp{Lec.\ Notes in Physics}
          % Lecture Notes in Physics
\def\cpc{Comp.\ Phys.\ Comm.}
          % Computer Physics Communications
\def\jpg{J. Phys. G}
          % Journal of Physics G Nuclear Physics
\def\ijmpa{Int.\ J.\ Mod.\ Phys.\ A}
          % International Journal of Modern Physics A
\def\epjc{Eur.\ Phys.\ J.\ C}
          % European Physical Journal C
\def\nima{Nuc.\ Inst.\ Methods A}
          % Nuclear Instruments and Methods A
\def\nimb{Nuc.\ Inst.\ Methods B}
          % Nuclear Instruments and Methods B
\def\njp{New J.\ Phys.}
          % New Journal of Physics
\def\rmp{Rev.\ Mod.\ Phys.}
          % Reviews of Modern Physics
\def\app{Astropart.\ Phys.}
          % Astroparticle Physics
\def\aj{AJ}%
          % Astronomical Journal
\def\actaa{Acta Astron.}%
          % Acta Astronomica
\def\araa{ARA\&A}%
          % Annual Review of Astron and Astrophys
\def\arnps{Ann.~Rev.~Nucl.~\& Part.~Sci.}%
          % Annual Review of Astron and Astrophys
\def\apj{ApJ}%
          % Astrophysical Journal
\def\apjl{ApJ}%
          % Astrophysical Journal, Letters
\def\apjs{ApJS}%
          % Astrophysical Journal, Supplement
\def\ao{Appl.\ Opt.}%
          % Applied Optics
\def\apss{Ap\&SS}%
          % Astrophysics and Space Science
\def\aap{A\&A}%
          % Astronomy and Astrophysics
\def\aapr{A\&A~Rev.}%
          % Astronomy and Astrophysics Reviews
\def\aaps{A\&AS}%
          % Astronomy and Astrophysics, Supplement
\def\azh{AZh}%
          % Astronomicheskii Zhurnal
\def\pos{PoS}%
          % Proceedings of Science
\def\baas{BAAS}%
          % Bulletin of the AAS
\def\bac{Bull.\ Astr.\ Inst.\ Czechosl.}%
          % Bulletin of the Astronomical Institutes of Czechoslovakia
\def\caa{Chinese Astron.\ Astrophys.}%
          % Chinese Astronomy and Astrophysics
\def\cjaa{Chinese J.\ Astron.\ Astrophys.}%
          % Chinese Journal of Astronomy and Astrophysics
\def\icarus{Icarus}%
          % Icarus
\def\jhep{JHEP}%
          % Journal of High Energy Physics
\def\jcap{JCAP}%
          % Journal of Cosmology and Astroparticle Physics
\def\jinst{JINST}%
          % Journal of Instrumentation
\def\jpsj{J.\ Phys.\ Soc.\ Japan}%
          % Journal of the Physical Society of Japan
\def\jrasc{JRASC}%
          % Journal of the RAS of Canada
\def\canjphys{Can.~J.~Phys.}
          %Canadian Journal of Physics
\def\apphys{Astropart.~Phys.}
          %Astroparticle Physics
\def\mnras{MNRAS}%
          % Monthly Notices of the RAS
\def\memras{MmRAS}%
          % Memoirs of the RAS
\def\na{New A}%
          % New Astronomy
\def\nar{New A Rev.}%
          % New Astronomy Review
\def\pasa{PASA}%
          % Publications of the Astron. Soc. of Australia
\def\pra{Phys.\ Rev.\ A}%
          % Physical Review A: General Physics
\def\prb{Phys.\ Rev.\ B}%
          % Physical Review B: Solid State
\def\prc{Phys.\ Rev.\ C}%
          % Physical Review C
\def\prd{Phys.\ Rev.\ D}%
          % Physical Review D
\def\pre{Phys.\ Rev.\ E}%
          % Physical Review E
\def\prx{Phys.\ Rev.\ X}%
          % Physical Review X
\def\prl{Phys.\ Rev.\ Lett.}%
          % Physical Review Letters
\def\pasp{PASP}%
          % Publications of the ASP
\def\pasj{PASJ}%
          % Publications of the ASJ
\def\qjras{QJRAS}%
          % Quarterly Journal of the RAS
\def\rmxaa{Rev. Mexicana Astron. Astrofis.}%
          % Revista Mexicana de Astronomia y Astrofisica
\def\skytel{S\&T}%
          % Sky and Telescope
\def\solphys{Sol.\ Phys.}%
          % Solar Physics
\def\sovast{Soviet~Ast.}%
          % Soviet Astronomy
\def\ssr{Space~Sci.\ Rev.}%
          % Space Science Reviews
\def\zap{ZAp}%
          % Zeitschrift fuer Astrophysik
\def\nat{Nature}%
          % Nature
\def\science{Science}%
\def\sci{\science}%
          % Science
\def\iaucirc{IAU~Circ.}%
          % IAU Cirulars
\def\aplett{Astrophys.\ Lett.}%
          % Astrophysics Letters
\def\apspr{Astrophys.\ Space~Phys.\ Res.}%
          % Astrophysics Space Physics Research
\def\bain{Bull.\ Astron.\ Inst.\ Netherlands}%
          % Bulletin Astronomical Institute of the Netherlands
\def\fcp{Fund.\ Cosmic~Phys.}%
          % Fundamental Cosmic Physics
\def\gca{Geochim.\ Cosmochim.\ Acta}%
          % Geochimica Cosmochimica Acta
\def\grl{Geophys.\ Res.\ Lett.}%
          % Geophysics Research Letters
\def\jcp{J.\ Chem.\ Phys.}%
          % Journal of Chemical Physics
\def\jgr{J.\ Geophys.\ Res.}%
          % Journal of Geophysics Research
\def\jqsrt{J.\ Quant.\ Spec.\ Radiat.\ Transf.}%
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer
\def\memsai{Mem.\ Soc.\ Astron.\ Italiana}%
          % Mem. Societa Astronomica Italiana
\def\nphysa{Nucl.\ Phys.\ A}%
          % Nuclear Physics A
\def\nphysb{Nucl.\ Phys.\ B}%
          % Nuclear Physics B
\def\physrep{Phys.\ Rep.}%
          % Physics Reports
\def\physscr{Phys.\ Scr}%
          % Physica Scripta
\def\planss{Planet.\ Space~Sci.}%
          % Planetary Space Science
\def\procspie{Proc.\ SPIE}%
          % Proceedings of the SPIE
\def\repprogphys{Rep.\ Prog.\ Phys.}%
          % Reports of Progress in Physics
\def\jpcrd{J. Phys. Chem. Ref. Data}%
        %Journal of Physical and Chemical Reference Data
\def\jphysb{J. Phys. B}%
	%Journal of Physics B Atomic Molecular Physics
\def\jphysd{J. Phys. D}%
	%Journal of Physics D
\def\jphysconfseries{J. Phys. Conf. Series}%
	%Journal of Physics: Conference Series
\def\physrev{\pr}
\def\pr{Phys. Rev.}%
	%Physical Review
\def\josa{J. Opt. Soc. Amer. (1917-1983)}%
	%Journal of the Optical Society of America (1917-1983)
\def\josab{J. Opt. Soc. Amer. B}%
	%Journal of the Optical Society of America B Optical Physics
\def\pla{Phys. Lett. A}%
	%Physics Letters A
\def\plb{Phys. Lett. B}%
	%Physics Letters B
\def\os{Opt. Spectrosc. (Russ.)}%
	%Optics and Spectroscopy (Russ. / USSR)
\def\jas{J. Appl. Spectrosc.}%
	%Journal of Applied Spectroscopy (Russ. / USSR)
\def\annp{Ann. Phys.}%
	%Annalen der Physik
\def\sa{Spectrochim. Acta}%
	%Spectrochimica Acta
\def\prsoca{Proc. R. Soc. London Ser. A}%
	%Proceedings of the Royal Society of London, Series A
\def\zphysa{Z. Phys. A}%
	%Zeitschrift fur Physik A
\def\zphysb{Z. Phys. B}%
	%Zeitschrift fur Physik B
\def\zphysc{Z. Phys. C}%
	%Zeitschrift fur Physik C
\def\zphysd{Z. Phys. D}%
	%Zeitschrift fur Physik D
\def\zphyse{Z. Phys. E}%
	%Zeitschrift fur Physik E
\def\zphys{Z. Phys.}%
	%Zeitschrift fur Physik
\def\adndt{Atom. Data Nuc. Data Tables}%
	%Atomic Data and Nuclear Data Tables
\def\jmolspec{J. Mol. Spectrosc.}%
	%Journal of Molecular Spectroscopy
\def\aphysb{Appl. Phys. B}%
	%Applied Physics B: Lasers and Optics
\def\nim{Nuc. Inst. Meth.}%
	%Nuclear Instruments and Methods
\def\jphysique{J. Phys. (Paris)}%
	%Journal de Physique
\def\epjp{Eur.~Phys.~J.~Plus}%
        %European Physical Journal Plus
\def\epjc{Eur.~Phys.~J.~C}%
        %European Physical Journal C
\def\epl{Europhys.~Lett}%
        %Europhysics Letters
\def\njp{New J.~Phys.}
        %New Journal of Physics
\def\statsci{StatSci}
\def\an{AstNach}
\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao
%


